Hybrid Beamforming for Large Antenna Arrays with Phase Shifter Selection

This paper proposes an asymptotically optimal hybrid beamforming solution for large antenna arrays by exploiting the properties of the singular vectors of the channel matrix. It is shown that the elements of the channel matrix with Rayleigh fading follow a normal distribution when large antenna arrays are employed. The proposed beamforming algorithm is effective in both sparse and rich propagation environments, and is applicable for both point-to-point and multiuser scenarios. In addition, a closed-form expression and a lower-bound for the achievable rates are derived when analog and digital phase shifters are employed. It is shown that the performance of the hybrid beamformers using phase shifters with more than 2-bits resolution is comparable with analog phase shifting. A novel phase shifter selection scheme that reduces the power consumption at the phase shifter network is proposed when the wireless channel is modeled by Rayleigh fading. Using this selection scheme, the spectral efficiency can be increased as the power consumption in the phase shifter network reduces. Compared to the scenario that all of the phase shifters are in operation, the simulation results indicate that the spectral efficiency increases when up to 50% of phase shifters are turned off.

==> StateOfTheArt_-_Copy.tex <==
\subsection{Discussion and Comparison with the State-of-the-art}
\label{StateofArt}
One of the common approaches in the literature is to decompose the unconstrained thin-SVD based beamformer matrix into RF beamformer and baseband precoder matrices, \cite{SpatiallySparsePrecodingAyach,SohailICC2015,NiDL15}. The computational complexity of the rank-$M$ thin-SVD of \textbf{H} is $O(N_\text{t} N_\text{r} M)$ for $M \ll \sqrt{N_\text{t} N_\text{r}}$ \cite{Brand200620}. The state-of-the-art hybrid beamformers that require a second round of computations to decompose $\textbf{F}_\text{d}$ into $\textbf{F}_\text{B}^\text{opt}$ and $\textbf{F}_\text{RF}^\text{opt}$ can cause high computational delay and complexity \cite{SpatiallySparsePrecodingAyach,SohailICC2015}. An iterative algorithm can be used to solve the optimization problem in (\ref{eq:OptimalJointDesign}), however, the iterative algorithm renders a high computational cost and delay \cite{PerAntennaPi2012,FoadTorontoApril2015Digital,NiDL15}. For example, the complexity of the hybrid beamformer in \cite{FoadTorontoApril2015} is $O(\max (N_\text{t},N_\text{r})^2 \min(N_\text{t},N_\text{r}))$. {\color{blue}{The computational complexity of the hybrid beamformer of Lemma 2 is equal to rank-$M$ thin-SVD which is $O(N_\text{t} N_\text{r} M)$. 

It should be noted that the hybrid beamformer of Lemma 2 for very large number of antennas is equivalent to beam steering for the geometry based channel. The reason is that when the transmitter and the receiver are equipped with uniform linear arrays with antenna spacing of $\lambda/2$, the singular vectors of the channel matrix follow the structure of discrete-Fourier transform (DFT) matrix \cite{DeconstructingMultiantennaSaeed}. In this case, the elements of the singular vectors are in the form of $\text{e}^{j\theta}$, and hence, $\textbf{F}_\text{RF}$ can be easily set towards the direction of the singular vectors. The advantage of the hybrid beamformers in \cite{SpatiallySparsePrecodingAyach,NiDL15,PerAntennaPi2012,FoadTorontoApril2015Digital} is that their design does not depend on the size of the array. Although the analysis in Subsection IV. B was focused on the asymptotically large antenna arrays, the proposed hybrid beamformer can achieve a close to optimal performance and the closed-forms can provide a good approximation even with relatively small number of antennas as it will be shown in Section \ref{sec:imulations}. 

Finally, the RF codebook based approaches are only applicable to a fixed type of channel and array structure such as sparse geometry based model \cite{SpatiallySparsePrecodingAyach,SohailICC2015}, and they are not applicable to other channels such as Rayleigh fading without a new codebook design. For the Rayleigh channel model, the proposed algorithm does not have any constraints on the array structure, and it does not require an RF codebook even with digital phase shifters. In addition, the closed-form expressions of the achievable rates for Rayleigh channel model are derived which to best of the authors' knowledge was not previously reported.The hybrid beamformer of Lemma 2, however, can be used in both channel models. Considering the performance for finite number of antennas and simplicity of the proposed hybrid beamformer for both rich and sparse scattering channels, it can be one of the candidate approaches to be implemented in low complexity hardware architectures. 
 }} 


